Energy Reduction in Cell-Free Massive MIMO through Fine-Grained Resource Management

The physical layer foundations of cell-free massive MIMO (CF-mMIMO) have been well-established. As a next step, researchers are investigating practical and energy-efficient network implementations. This paper focuses on multiple sets of access points (APs) where user equipments (UEs) are served in each set, termed a federation, without inter-federation interference. The combination of federations and CF-mMIMO shows promise for highly-loaded scenarios. Our aim is to minimize the total energy consumption while adhering to UE downlink data rate constraints. The energy expenditure of the full system is modelled using a detailed hardware model of the APs. We jointly design the AP-UE association variables, determine active APs, and assign APs and UEs to federations. To solve this highly combinatorial problem, we develop a novel alternating optimization algorithm. Simulation results for an indoor factory demonstrate the advantages of considering multiple federations, particularly when facing large data rate requirements. Furthermore, we show that adopting a more distributed CF-mMIMO architecture is necessary to meet the data rate requirements. Conversely, if feasible, using a less distributed system with more antennas at each AP is more advantageous from an energy savings perspective.

==> results/fig-30-60-120-CSPs.tex <==
\begin{figure}
    \centering
    
\begin{tikzpicture}[spy using outlines={rectangle, magnification=2, connect spies}]

    \begin{axis}[
        ylabel={Consumed Power (\si{\kilo\watt})},
        xlabel={Data Rate (\si{\mega\bit\per\second})},
        width=0.7\linewidth, % Set the width of the plot
        minor x tick num=3,
        %clip=false,
        minor y tick num=4,
        legend columns=3,
        cycle list/Dark2,
        legend style={nodes={scale=0.8, transform shape}},
        legend style={at={(0.5,1.02)},anchor=south},
        grid=major,
        %ylabel near ticks,
        %axis y line*=right,
        %y axis line style={red},
        %hide x axis,
        % every y axis label/.append style ={red},
        % every y tick label/.append style={red},
         xmin=10, xmax=86,
        ymin=-0.099, ymax=1.399, % Adjust these values according to your data
        % ytick={0,3,6,9},
        % yticklabels={0,3,6,9},
    ]
    \pgfplotstableread{results/power-factory.txt}\myenergydata;

    % Factory data
    \addplot+[mark=*, mark size=1pt] table [x=data-rate, y=factory-30,  y expr=\thisrow{factory-30}/1000] {\myenergydata};
    \addlegendentry{30 CSPs}

     % Factory data
    \addplot+[mark=square*, mark size=1pt] table [x=data-rate, y=factory-60,  y expr=\thisrow{factory-60}/1000] {\myenergydata};
    \addlegendentry{60 CSPs}


    \addplot+[mark=triangle*, mark size=1pt] table [ x=data-rate, y=factory-120,  y expr=\thisrow{factory-120}/1000] {\myenergydata};
    \addlegendentry{120 CSPs}



     %\node[label={\scriptsize 30 \glspl{csp}}, anchor=south west] at (axis cs:90,1) {};
      \addplot[mark=none, forget plot, dashed] coordinates {(10,0.3085) (86,0.3085)};
      

      \node[label={\scriptsize 60 \glspl{csp}}, anchor=south west] at (axis cs:40,48) {};
       \addplot[mark=none, forget plot, dashed] coordinates {(10,0.61467) (86,0.61467)};
      
       \node[label={\scriptsize 120 \glspl{csp}}, anchor=south west] at (axis cs:40,48) {};
        \addplot[mark=none, forget plot, dashed] coordinates {(10,1.22699) (86,1.22699)};

    % Spy scope
    \coordinate (spypoint) at (axis cs:20,0.120);
    \coordinate (magnifyglass) at (axis cs:35,0.9);

    \end{axis}
    
    \spy [red, size=1.2cm, magnification=3] on (spypoint) in node at (magnifyglass);
    \end{tikzpicture}
    \caption{\gilles{TODO}}
    \label{fig:results}
\end{figure}
